On the Fidelity Distribution of Link-level Entanglements under Purification

Quantum entanglement is the key to quantum communications over considerable distances. The first step for entanglement distribution among quantum communication nodes is to generate link-level Einstein-Podolsky-Rosen (EPR) pairs between adjacent communication nodes. EPR pairs may be continuously generated and stored in a few quantum memories to be ready for utilization by quantum applications. A major challenge is that qubits suffer from unavoidable noise due to their interaction with the environment, which is called decoherence. This decoherence results in the known exponential decay model of the fidelity of the qubits with time, thus, limiting the lifetime of a qubit in a quantum memory and the performance of quantum applications. In this paper, we evaluate the fidelity of the stored EPR pairs under two opposite dynamical and probabilistic phenomena, first, the aforementioned decoherence and second purification, i.e. an operation to improve the fidelity of an EPR pair at the expense of sacrificing another EPR pair. Instead of applying the purification as soon as two EPR pairs are generated, we introduce a Purification scheme Beyond the Generation time (PBG) of two EPR pairs. We analytically show the probability distribution of the fidelity of stored link-level EPR pairs in a system with two quantum memories at each node allowing a maximum of two stored EPR pairs. In addition, we apply a PBG scheme that purifies the two stored EPR pairs upon the generation of an additional one. We finally provide numerical evaluations of the analytical approach and show the fidelity-rate trade-off of the considered purification scheme.

==> Figs_1/CDF_per_qubit.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=2.5in,
height=1in,
scale only axis,
xmin=0.5,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={Fidelity},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={CDF},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
legend pos=north west
]
\draw[line width=0.005 \linewidth](current axis.south west)rectangle(current axis.north east);
\addplot[const plot, color=red] table[row sep=crcr] {%
0.548891722025675	0.0044179178581204\\
0.552699612280932	0.00534628283457528\\
0.556804076835382	0.00646809106785418\\
0.561228214126491	0.00782323959800196\\
0.565996921593915	0.0094597503734227\\
0.571137035793257	0.0114353983966659\\
0.576677483422464	0.0138196592940273\\
0.582649444110793	0.0166960371801665\\
0.589086525886449	0.020164844807104\\
0.596024954310377	0.024346521002812\\
0.603503776340576	0.0293855856037171\\
0.611565080074215	0.0352824624840817\\
0.620254231604171	0.042325434810492\\
0.629620130322946	0.0507309578696312\\
0.639715484110704	0.0607536872778361\\
0.650597105956101	0.0726581570696193\\
0.662326233679175	0.0868055455347206\\
0.674968874555578	0.103618636971368\\
0.688596176781578	0.123554223731252\\
0.7032848298703	0.147180010828297\\
0.719117496232475	0.175132337288939\\
0.736183276370507	0.208128989166012\\
0.754578210303775	0.246977096795225\\
0.774405818047013	0.292631092394893\\
0.795777682183407	0.346152376773249\\
0.818814075810887	0.408179826687562\\
0.843644639395486	0.480291673370372\\
0.870409110340859	0.563483643791583\\
0.899258109379689	0.657777517137321\\
0.930353988212529	0.764224249982465\\
0.963871743164276	0.880687082830104\\
1	1\\
};
\addlegendentry{Analyt.}

% \addplot[const plot, color=black] table[row sep=crcr] {%
% 0.548891722025675	0.013292\\
% 0.552699612280932	0.0158765\\
% 0.556804076835382	0.018952\\
% 0.561228214126491	0.02262\\
% 0.565996921593915	0.0269765\\
% 0.571137035793257	0.032159\\
% 0.576677483422464	0.038315\\
% 0.582649444110793	0.045612\\
% 0.589086525886449	0.054194\\
% 0.596024954310377	0.0642835\\
% 0.603503776340576	0.0761725\\
% 0.611565080074215	0.0900955\\
% 0.620254231604171	0.106348\\
% 0.629620130322946	0.1252325\\
% 0.639715484110704	0.147074\\
% 0.650597105956101	0.1723645\\
% 0.662326233679175	0.2014265\\
% 0.674968874555578	0.234735\\
% 0.688596176781578	0.2727315\\
% 0.7032848298703	0.3158015\\
% 0.719117496232475	0.364385\\
% 0.736183276370507	0.418496\\
% 0.754578210303775	0.478492\\
% 0.774405818047013	0.544005\\
% 0.795777682183407	0.6145065\\
% 0.818814075810887	0.688575\\
% 0.843644639395486	0.764652\\
% 0.870409110340859	0.83957\\
% 0.899258109379689	0.908502\\
% 0.930353988212529	0.965078\\
% 0.963871743164276	1\\
% 1	1\\
% };
% \addlegendentry{No Pur.}

\addplot[const plot, color=blue, draw=none, only marks, mark=o, mark options={solid, blue}] table[row sep=crcr] {%
0.548891722025675	0.0044535\\
0.552699612280932	0.0053995\\
0.556804076835382	0.00654\\
0.561228214126491	0.0079065\\
0.565996921593915	0.0095675\\
0.571137035793257	0.0115635\\
0.576677483422464	0.0139655\\
0.582649444110793	0.016858\\
0.589086525886449	0.020345\\
0.596024954310377	0.0245715\\
0.603503776340576	0.029644\\
0.611565080074215	0.0355965\\
0.620254231604171	0.0427155\\
0.629620130322946	0.051198\\
0.639715484110704	0.0612565\\
0.650597105956101	0.0731925\\
0.662326233679175	0.087414\\
0.674968874555578	0.1043625\\
0.688596176781578	0.1244295\\
0.7032848298703	0.1481915\\
0.719117496232475	0.1763345\\
0.736183276370507	0.20947\\
0.754578210303775	0.248476\\
0.774405818047013	0.2942165\\
0.795777682183407	0.3478445\\
0.818814075810887	0.409881\\
0.843644639395486	0.4819335\\
0.870409110340859	0.5649075\\
0.899258109379689	0.658862\\
0.930353988212529	0.7648925\\
0.963871743164276	0.8808955\\
1	1\\
};
\addlegendentry{Sim.}

% \addplot[const plot, color=red, dashed] table[row sep=crcr] {%
% 0.548891722025675	0.183430928381452\\
% 0.552699612280932	0.18374195032717\\
% 0.556804076835382	0.18412432161086\\
% 0.561228214126491	0.184594409977948\\
% 0.565996921593915	0.185172337982211\\
% 0.571137035793257	0.18588284434973\\
% 0.576677483422464	0.186756342942219\\
% 0.582649444110793	0.187830224649636\\
% 0.589086525886449	0.189150457940725\\
% 0.596024954310377	0.190773556584515\\
% 0.603503776340576	0.192768998772844\\
% 0.611565080074215	0.195222201196613\\
% 0.620254231604171	0.19823817538378\\
% 0.629620130322946	0.201946022811912\\
% 0.639715484110704	0.206504461212613\\
% 0.650597105956101	0.212108618626246\\
% 0.662326233679175	0.218998386032547\\
% 0.674968874555578	0.227468686098966\\
% 0.688596176781578	0.23788209760972\\
% 0.7032848298703	0.250684375975536\\
% 0.719117496232475	0.266423534193436\\
% 0.736183276370507	0.285773301034121\\
% 0.754578210303775	0.3095619606057\\
% 0.774405818047013	0.338807807797132\\
% 0.795777682183407	0.374762737303395\\
% 0.818814075810887	0.418965832099671\\
% 0.843644639395486	0.473309245267211\\
% 0.870409110340859	0.54011919530145\\
% 0.899258109379689	0.622255541979131\\
% 0.930353988212529	0.723234205218645\\
% 0.963871743164276	0.847377667182604\\
% 1	1\\
% };
% \addlegendentry{data4}

% \addplot[const plot, color=black, dashed] table[row sep=crcr] {%
% 0.548891722025675	0.001606\\
% 0.552699612280932	0.0019875\\
% 0.556804076835382	0.002452\\
% 0.561228214126491	0.003012\\
% 0.565996921593915	0.0037115\\
% 0.571137035793257	0.0045525\\
% 0.576677483422464	0.005586\\
% 0.582649444110793	0.006877\\
% 0.589086525886449	0.008475\\
% 0.596024954310377	0.0104555\\
% 0.603503776340576	0.0129025\\
% 0.611565080074215	0.0159005\\
% 0.620254231604171	0.019602\\
% 0.629620130322946	0.0241495\\
% 0.639715484110704	0.0298075\\
% 0.650597105956101	0.0367355\\
% 0.662326233679175	0.0452315\\
% 0.674968874555578	0.055667\\
% 0.688596176781578	0.068523\\
% 0.7032848298703	0.084313\\
% 0.719117496232475	0.1036215\\
% 0.736183276370507	0.1273905\\
% 0.754578210303775	0.156496\\
% 0.774405818047013	0.192254\\
% 0.795777682183407	0.2362675\\
% 0.818814075810887	0.290407\\
% 0.843644639395486	0.3567975\\
% 0.870409110340859	0.438367\\
% 0.899258109379689	0.538761\\
% 0.930353988212529	0.6620755\\
% 0.963871743164276	0.813577\\
% 1	1\\
% };
% \addlegendentry{data5}

% \addplot[const plot, color=blue, draw=none, only marks, mark=*, mark options={solid, blue}] table[row sep=crcr] {%
% 0.548891722025675	0.1848855\\
% 0.552699612280932	0.185184\\
% 0.556804076835382	0.1855695\\
% 0.561228214126491	0.1860355\\
% 0.565996921593915	0.1866045\\
% 0.571137035793257	0.1873035\\
% 0.576677483422464	0.188166\\
% 0.582649444110793	0.1892295\\
% 0.589086525886449	0.1905425\\
% 0.596024954310377	0.192164\\
% 0.603503776340576	0.1941355\\
% 0.611565080074215	0.196588\\
% 0.620254231604171	0.1996145\\
% 0.629620130322946	0.2033355\\
% 0.639715484110704	0.2078895\\
% 0.650597105956101	0.213527\\
% 0.662326233679175	0.2204215\\
% 0.674968874555578	0.2289385\\
% 0.688596176781578	0.23941\\
% 0.7032848298703	0.2522735\\
% 0.719117496232475	0.2681255\\
% 0.736183276370507	0.2875945\\
% 0.754578210303775	0.3114395\\
% 0.774405818047013	0.340741\\
% 0.795777682183407	0.376731\\
% 0.818814075810887	0.4208875\\
% 0.843644639395486	0.4750645\\
% 0.870409110340859	0.541545\\
% 0.899258109379689	0.623392\\
% 0.930353988212529	0.724006\\
% 0.963871743164276	0.847718\\
% 1	1\\
% };
% \addlegendentry{data6}

\end{axis}

\end{tikzpicture}%

==> Figs_1/Fidelity_av.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=1.9 in,
height=0.8 in,
scale only axis,
xmin=0,
xmax=30,
xlabel style={font=\color{white!15!black}},
xlabel={},
ymin=0.5,
ymax=0.9,
ylabel style={font=\color{white!15!black}},
ylabel={Average fidelity},
 xlabel style={yshift=0.2cm},
 ylabel style={yshift=-0.2cm},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=center, draw=white!15!black},
legend pos=outer north east
]
\draw[line width=0.005 \linewidth](current axis.south west)rectangle(current axis.north east);
\addplot [color=red, dashed, mark=asterisk, mark options={solid, red}]
  table[row sep=crcr]{%
4	0.866581814229352\\
6	0.855502089793015\\
8	0.843542439912428\\
10	0.830626572512208\\
12	0.816625323268054\\
14	0.801312451625456\\
16	0.784692436011012\\
18	0.767216433037433\\
20	0.74890244550562\\
22	0.7326911910752\\
24	0.71532447914742\\
26	0.703117972474478\\
28	0.690670366474805\\
30	0.681114912060855\\
};
\addlegendentry{$\bar{F}_1$ }

% \addplot [color=blue, mark=asterisk, mark options={solid, blue}]
%   table[row sep=crcr]{%
% 4	0.866559213625909\\
% 6	0.855324186234592\\
% 8	0.843472928718789\\
% 10	0.830428128735889\\
% 12	0.816180617106229\\
% 14	0.801532852402089\\
% 16	0.784926498903304\\
% 18	0.767048275299573\\
% 20	0.748990134057874\\
% 22	0.732297998429549\\
% 24	0.715177791458992\\
% 26	0.704364936162796\\
% 28	0.691140134674263\\
% 30	0.680328560558129\\
% };
% \addlegendentry{data2}

\addplot [color=black,dashed, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
4	0.862020312967795\\
6	0.847587444925506\\
8	0.832053955879811\\
10	0.813457574830884\\
12	0.79301352648292\\
14	0.771467241170564\\
16	0.747181132645771\\
18	0.723782841362235\\
20	0.697917484408851\\
22	0.676455787355103\\
24	0.654872445895799\\
26	0.639357876214099\\
28	0.6246358889794\\
30	0.614009000658454\\
};
\addlegendentry{$\bar{F}_1$ no Pur. }

\addplot [color=red, mark=asterisk, mark options={solid, red}]
  table[row sep=crcr]{%
4	0.854646777752017\\
6	0.8342667885601\\
8	0.810999095627159\\
10	0.784184942016211\\
12	0.754095719257302\\
14	0.72255058911743\\
16	0.690631774197472\\
18	0.659338286265096\\
20	0.632333006618793\\
22	0.613419823946532\\
24	0.595903866966085\\
26	0.588199810909552\\
28	0.580607412862135\\
30	0.577218117001324\\
};
\addlegendentry{$\bar{F}_2$}

% \addplot [color=blue, mark=o, mark options={solid, blue}]
%   table[row sep=crcr]{%
% 4	0.854466502201283\\
% 6	0.834120697821871\\
% 8	0.811280262952613\\
% 10	0.784320528555878\\
% 12	0.754097759634589\\
% 14	0.722396838839044\\
% 16	0.691081998688227\\
% 18	0.659182986411076\\
% 20	0.632377914863486\\
% 22	0.613592686341992\\
% 24	0.595574191805898\\
% 26	0.58842286574077\\
% 28	0.580972344740875\\
% 30	0.577127638969313\\
% };
% \addlegendentry{data5}

\addplot [color=black, mark=o, mark options={solid, black}]
  table[row sep=crcr]{%
4	0.725811007274639\\
6	0.707811807480964\\
8	0.689666875862282\\
10	0.669233314740845\\
12	0.648095250086856\\
14	0.627450617190873\\
16	0.607119115946495\\
18	0.590450695253913\\
20	0.575719424309167\\
22	0.56802464040399\\
24	0.559830187927537\\
26	0.558778165353851\\
28	0.556947689786336\\
30	0.557832572118856\\
};
\addlegendentry{$\bar{F}_2$ no Pur.}

\end{axis}

\end{tikzpicture}%

==> Figs_1/average_qubits_nr.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=1.9in,
height=0.8in,
scale only axis,
xmin=0,
xmax=30,
xlabel style={font=\color{white!15!black}},
xlabel={Distance (\si{\km})},
ymin=0.5,
ymax=2,
ylabel style={font=\color{white!15!black}},
ylabel={Average Nr. of qubits},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
 xlabel style={yshift=0.2cm},
 ylabel style={yshift=-0.35cm},
legend style={legend cell align=left, align=center, draw=white!15!black},
legend pos= outer north east
]
\draw[line width=0.005 \linewidth](current axis.south west)rectangle(current axis.north east);
\addplot [color=red, mark=asterisk, mark options={solid, red}]
  table[row sep=crcr]{%
4	1.96137991553602\\
6	1.93877226233881\\
8	1.91416626517407\\
10	1.88767463381145\\
12	1.85955870744601\\
14	1.82926335782253\\
16	1.79192955689493\\
18	1.73745732619102\\
20	1.6614281449156\\
22	1.53046435348412\\
24	1.39801151841903\\
26	1.2121473417878\\
28	1.03745130998936\\
30	0.865457082078241\\
};
\addlegendentry{Pur. \\(Analyt.)}

% \addplot [color=blue, dashed, mark=o, mark options={solid, blue}]
%   table[row sep=crcr]{%
% 4	1.961132\\
% 6	1.93848\\
% 8	1.915051\\
% 10	1.8884565\\
% 12	1.8605835\\
% 14	1.8280375\\
% 16	1.792243\\
% 18	1.7369015\\
% 20	1.660011\\
% 22	1.5306615\\
% 24	1.3946505\\
% 26	1.212544\\
% 28	1.041894\\
% 30	0.8634535\\
% };
% \addlegendentry{Sim}

\addplot [color=black, mark=square, mark options={solid, black}]
  table[row sep=crcr]{%
4	1.999999\\
6	2\\
8	1.999996\\
10	1.999967\\
12	1.9990625\\
14	1.99245\\
16	1.969115\\
18	1.916966\\
20	1.82631\\
22	1.6558375\\
24	1.4988675\\
26	1.2681635\\
28	1.0692235\\
30	0.875932\\
};
\addlegendentry{No Pur. \\ (Sim.)}

\end{axis}
\end{tikzpicture}%
